Blink: Lightweight Sample Runs for Cost Optimization of Big Data Applications

Distributed in-memory data processing engines accelerate iterative applications by caching substantial datasets in memory rather than recomputing them in each iteration. Selecting a suitable cluster size for caching these datasets plays an essential role in achieving optimal performance. In practice, this is a tedious and hard task for end users, who are typically not aware of cluster specifications, workload semantics and sizes of intermediate data. We present Blink, an autonomous sampling-based framework, which predicts sizes of cached datasets and selects optimal cluster size without relying on historical runs. We evaluate Blink on a variety of iterative, real-world, machine learning applications. With an average sample runs cost of 4.6% compared to the cost of optimal runs, Blink selects the optimal cluster size in 15 out of 16 cases, saving up to 47.4% of execution cost compared to average costs.

==> sections/acknowledgments.tex <==
% !TeX spellcheck = en_US
%-------------------------------------------------------------------------------
% Acknowledgments
%-------------------------------------------------------------------------------

\begin{acks}

To..

\end{acks}

%-------------------------------------------------------------------------------
% Commented part below.
%-------------------------------------------------------------------------------



==> sections/discussion.tex <==
% !TeX spellcheck = en_US
%-------------------------------------------------------------------------------
\section{Discussion}
\label{sec:discussion}
%-------------------------------------------------------------------------------
 
\revision{TODO Hani}

%-------------------------------------------------------------------------------
% Commented part below.
%-------------------------------------------------------------------------------



==> sections/implementation.tex <==
% !TeX spellcheck = en_US
%-------------------------------------------------------------------------------
\section{Implementation}
\label{sec:implementation}
%-------------------------------------------------------------------------------



%-------------------------------------------------------------------------------
% Commented part below.
%-------------------------------------------------------------------------------



==> sections/zoom-in.tex <==
% !TeX spellcheck = en_US
%-------------------------------------------------------------------------------
\section{Zoom-in}
\label{sec:zoom-in}
%-------------------------------------------------------------------------------

Here it follows a small intro about the section.. 

\subsection{Size prediction error}
\label{subsec:size-prediction-error}

Herein, we discuss size prediction accuracy of \textsc{gbt} (\SI{63.3}{\percent}). 
To get better insights, we additionally run 7 sample experiments with new data scales (\SIrange{0.4}{1.0}{\percent}). 
Figure~\ref{fig:gbt-sampling-cost-vs-prediction-accuracy-ratio} shows a sampling cost increment and prediction improvement in \textsc{gbt}. 
From this we can observe that prediction accuracy improves when we add more sampling experiments. 
For 10 sample runs, prediction accuracy is \SI{98.9}{\percent}. 
This proves that the poor prediction accuracy of cached intermediate results size in Section~\ref{subsec:prediction-accuracy-of-cached-intermediate-results} is not caused by the used model (Equation~\ref{eq:size-prediction}), but as a consequence of insufficient sample runs. 
However, by simply adding more sample runs, this does not necessarily improve efficiency. 
For example, by using 4 experiments, prediction accuracy reaches \SI{86.7}{\percent}, while it drops to \SI{73.5}{\percent} after the fifth experiment. 
The newly added experiment increases sampling cost to \SI{38.9}{\percent} and reduces prediction accuracy by \SI{13.2}{\percent}.

\begin{figure}[t!]
\centering
\input{figures/gbt-sampling-cost-vs-prediction-accuracy-ratio}
\vspace{-20pt}
\caption{Sampling cost and prediction accuracy of \textsc{gbt} with multiple experiments.}
\vspace{-15pt}
\label{fig:gbt-sampling-cost-vs-prediction-accuracy-ratio}
\end{figure}

We select prediction accuracy to sampling cost ratio to measure the benefit of adding more experiment/s.
Figure~\ref{fig:gbt-benefit} shows that conducting 4 experiments is the most efficient. 
However, by using 3 sample runs, \papertitle{} is able to select minimal required cluster configuration to cache intermediate results, in spite of data size prediction error, as shown in Section~\ref{subsec:optimal-configuration-selection}. 
Finally, as an explanation for the poor accuracy in \textsc{gbt}, the size of actual data in \textsc{gbt} is \SI{30.6}{\mega\byte}.
Therefore, during the process of running 3 sample runs, the training data is only few kilobytes, whereas the parallelism level is 100 (using \bsize{} sampling approach). 

\begin{figure}[t!]
\centering
\input{figures/gbt-benefit}
\vspace{-10pt}
\caption{Prediction accuracy vs. sampling cost ratio of \textsc{gbt}.}
\vspace{-15pt}
\label{fig:gbt-benefit}
\end{figure}

Figure~\ref{fig:gbt-data-size} shows the size of cached intermediate results in small data scales that are used to train size prediction models. 
Since \emph{cross validation} is used to evaluate size prediction models, it is worth mentioning that when we use 3 experiments, we get a model error of \SI{53.9}{\percent}. While with 10 experiments, we only get an error of \SI{28.5}{\percent}.
This error rate can be known before running actual runs.
Consequently, \papertitle{} can (as a future work) rely on it to perform additional sample runs, which would improve model accuracy and enhance outlier detection, by applying adaptive sampling.

\begin{figure}[t!]
\centering
\input{figures/gbt-data-size}
\vspace{-10pt}
\caption{Size of cached intermediate results of \textsc{gbt} during sample runs.}
\vspace{-15pt}
\label{fig:gbt-data-size}
\end{figure}
\if 0
\subsection{Selected cluster configuration in \textsc{svm}}

The selected cluster configuration for \textsc{svm} (i.e., 7 machines) was not the minimal cost one. The minimal cost configuration was 6 machines. Even though the error penalty was just 0.3 machines minutes (+\SI{0.4}{\percent}), but it was not expected since \papertitle{} selected the minimal required number of machines to cache intermediate results in memory without evictions. This exceptional case gave us the opportunity to conclude that selecting cluster configuration to fit intermediate results might not be always the major factor, as it was for the remaining 7 applications. 
\fi

\subsection{Data sample reduction}
\label{subsec:data-sample-reduction}

After proving the efficiency of \papertitle{} based on our experimental evaluations that rely on 3 tiny sample runs (\SI{0.1}{\percent} - \SI{0.3}{\percent}), we now evaluate the extent to which we can rely on \papertitle{}. 
The main questions we want to answer here are: 
\emph{Will \papertitle{} still be effective when we use smaller sample data scales (lower than \SI{0.1}{\percent})?} 
\emph{Can we relay on the same extracted size prediction models when actual data becomes larger (more than \SI{100}{\percent})?} 
To answer these questions, we apply \papertitle{} on larger actual data sets (i.e., \SI{150}{\percent} - \SI{18e4}{\percent} instead of \SI{100}{\percent}) and rely on the same extracted size prediction models used in Section~\ref{sec:evaluation}. 
As an exception, we rely on 10 sample runs for \textsc{gbt} (cf.~Section~\ref{subsec:size-prediction-error}). 
For the remaining applications, 3 sample runs are used. Table~\ref{tbl:application-details-ex} shows in details the overall analysis.

\input{tables/extended-evaluation}

\smallskip

\noindent \textbf{K-means.} 
As shown in Table~\ref{tbl:application-details-ex}, \papertitle{} selects 7 machines for \textsc{km} (which costs \SI{104.3}{} machine minutes) instead of 8 machines (which is the optimal configuration, with a cost of \SI{36.4} machine minutes). 
We realize that \papertitle{} predicts the size of cached intermediate results with high accuracy (\SI{99.7}{\percent}). 
The reason behind this suboptimal selected configuration is the unequal distribution of tasks among machines. 
The application parallelism is 100 and the number of recommended machines is 7, thus, the capacity of each machine is 14 tasks. 
However, some machines run more than 14 tasks and therefore some cached data partitions get evicted. 
Figure~\ref{fig:TasksDistribution-KMeans} illustrates the distribution of tasks in \textsc{km} on 7 machines. 
Herein, we observe that 7 cached data partitions are evicted from memory, which is the same number of tasks that are over-assigned to machines (15 tasks in machine $6 (+1)$, 16 tasks in machine $3 (+2)$, 16 tasks in machine $4 (+2)$, 16 tasks in machine $7 (+2))$. 
Finally, we realize that data partitions are equal in terms of size. 
However, it is important to highlight that in some cases of processing sparse data with non-optimal data partitioning, the size of data partitions varies. 
Hence, this might also affect the efficiency of \papertitle{}.

\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{figures/TasksDistribution-KMeans.png}
    \caption{Tasks distribution among machines in \textsc{km}}
    \vspace{-15pt}
    \label{fig:TasksDistribution-KMeans}
\end{figure}


==> sections/zoom-out.tex <==
% !TeX spellcheck = en_US
%-------------------------------------------------------------------------------
\section{Zoom-out}
\label{sec:zoom-out}
%-------------------------------------------------------------------------------

Here it follows a small intro about the section.. 

\subsection{Sampling overhead}
\label{subsec:sampling-overhead}

To evaluate the sampling overhead, we compare the sampling cost with the cost of actual runs when an optimal cluster configuration is selected. 
Figure~\ref{fig:sampling-to-optimal-cost-ratio} shows that on average, a sampling phase costs \SI{8.1}{\percent} of the total cost of an optimal actual run. 
At worst, the overhead is \SI{21.3}{\percent} (i.e., in \textsc{als}) while at best, it is \SI{1.6}{\percent} (i.e., in \textsc{rfc}).

\begin{figure}[t!]
\centering
\input{figures/sampling-vs-optimal-cost-ratio}
\vspace{-5pt}
\caption{\papertitle{} sampling versus optimal run: Cost ratio.}
\vspace{-15pt}
\label{fig:sampling-to-optimal-cost-ratio}
\end{figure}

By studying each sampling approach separately, we see that the average sampling cost of \bnumber{} is \SI{2.7}{\percent} -- with a worst case of \SI{5.1}{\percent} in \textsc{bayes} and a best case of \SI{1.6}{\percent} in \textsc{rfc}. 
For \bsize{}, the average sampling cost is \SI{13.3}{\percent} -- with a worst case of \SI{21.3}{\percent} in \textsc{als} and a best case of \SI{8.6}{\percent} in \textsc{km}. 
Altogether, \bsize{} costs about $ 4.9\times $ more than \bnumber{}. 
Nonetheless, the cost of \bsize{} is still tolerable because we are comparing these sampling costs with costs of optimal actual runs (which are minimal). 

By considering a selected cluster configuration for optimal runs by \papertitle{}, we can realize that the highest sampling costs are in \textsc{als}, \textsc{gbt}, and \textsc{pca}. 
An optimal configuration of all these applications is running on a single machine. 
In other words, a cost of actual runs does not include the number of machines as a factor.
This leads to high ratio numbers compared with sample runs, which also take place in a same cluster configuration. 
Finally, by taking \textsc{gbt} as an example of low cost actual run (\SI{9.7}{\minute} on a single machine; cf.~Table~\ref{tbl:application-details}), we still see the efficiency of \papertitle{} which costs \SI{14.4}{\percent} even with \bsize{}. 
In other words, \papertitle{} is still efficient for low-cost (i.e., short-running) applications.

\subsection{Prediction accuracy of size of cached intermediate results}
\label{subsec:prediction-accuracy-of-cached-intermediate-results}

We analyze the runtime logs of actual runs in order to get the size of cached intermediate results and compare them with the predicted size, based on 3 tiny sample runs (\SIrange{0.1}{0.3}{\percent}) and the size prediction model of Section~\ref{subsec:data-size-prediction}.
Figure~\ref{fig:size-prediction} indicates the error of \papertitle{} in predicting the size of cached intermediate results for each application. 
On average, the error was \SI{7.4}{\percent}.
We observe the best case in \textsc{svm} (\SI{0.0008}{\percent}) and the worst case in \textsc{gbt} (\SI{36.7}{\percent}). 
With the exception of \textsc{gbt}, we see the high accuracy of \papertitle{}, with higher than \SI{85}{\percent} in \textsc{als} and \SI{95}{\percent} in all remaining applications. 

\begin{figure}[t!]
\centering
\input{figures/prediction-error}
\vspace{-5pt}
\caption{\papertitle{} prediction error of cached intermediate result size.}
\vspace{-15pt}
\label{fig:size-prediction}
\end{figure}

%From this we can conclude that even though we only run 3 tiny sample runs (\SIrange{0.1}{0.3}{\percent}) and use a simple model (Equation~\ref{eq:size-prediction}), in all cases the prediction accuracy of cached intermediate result size in \papertitle{} is higher than \SI{90}{\percent}.

\subsection{Optimal configuration selection}
\label{subsec:optimal-configuration-selection}

We consider an optimal configuration as the minimum number of allocated machines that cache all intermediate results in memory without cache eviction. 
The green-colored cells in Table~\ref{tbl:application-details} indicate configurations where no eviction is required, while the bold numbers indicate optimal configurations recommended by \papertitle{} for each application. 
Table~\ref{tbl:application-details} shows that for all applications, \if 0, excluding \textsc{rfc},\fi  \papertitle{} selects a minimal number of machines required to cache intermediate results.
We can easily observe this by a comparison between a first green-colored cell and bold numbers of each application.

\input{tables/evaluation}
\if 0
During the analysis of our results, we observe an exceptional case in \textsc{svm}: notwithstanding the fact that \papertitle{} recommends an optimal solution with respect to caching all intermediate results in a minimal number of cluster configuration, the execution cost of the recommended cluster configuration is not the minimal. 
\fi
%Section~\ref{sec:discussion} covers in detail this case.

\if 0
During the analysis of our results, we observe two exceptional cases. 
The first case is related to \textsc{rfc}, whereby \papertitle{} recommends 4 machines, where on the contrary, it seems that cached intermediate results fit into memory of a single machine. 
The second case is related to \textsc{als}, whereby even if \papertitle{} recommends an optimal solution with respect to caching all intermediate results in a minimal amount of cluster configuration, however, execution cost of the recommended cluster configuration is not the minimal. 
This case is also similar in \textsc{svm}, having a negligible penalty.
Section~\ref{sec:discussion} covers in detail both the cases.
\fi

\subsection{Cost optimization}
\label{subsec:cost-optimization}

To evaluate the efficiency of \papertitle{}, we compare \papertitle{} cost with an average and worst cost of actual runs. 
\papertitle{} cost is the sum of sample run cost and actual run cost with a selected configuration by \papertitle{}. 
Figure~\ref{fig:blink-cost} shows that compared with an average cost, \papertitle{} saves \SI{40.6}{\percent} of execution cost, and compared with a worst case, it saves \SI{70.8}{\percent} of execution cost.

\begin{figure}[t!]
\centering
\input{figures/cost-optimization}
\vspace{-20pt}
\caption{\papertitle{} cost optimization.}
\vspace{-15pt}
\label{fig:blink-cost}
\end{figure}


==> tables/ClusterConfiguration.tex <==

\begin{table}[tb]
\centering
\small{
\npdecimalsign{.}
\nprounddigits{2}
\caption{Cost and time ratio of related components compared to \papertitle{}: Recommended cluster configuration.}
\label{tbl:evaluation-cluster-configuration}
\vspace{-10pt}
\begin{tabular}{ l r r }
\toprule
 & RelM & Ernest \\
\midrule
 Cost & \SI{96}{\percent} & \SI{258}{\percent}  \\
 Time & \SI{-59}{\percent}  & \SI{808}{\percent} \\
\bottomrule
\end{tabular}
\vspace{-10pt}
}
\end{table}


==> tables/extended-evaluation.tex <==

\begin{table*}[tb]
\centering
\small{
\npdecimalsign{.}
\nprounddigits{2}
\caption{Overview of evaluated \hibench{} applications. Recommended configuration is shown in bold.\\ Colored cells refer to configuration that do not cause cache evictions at all (all data partitions of intermediate results are fetched from memory). \\ x refers to failures caused by memory limitation.\\ Time unit is represented in minutes. Cost unit is represented in machine minutes.}
\vspace{-5pt}
\label{tbl:application-details-ex}
% \begin{tabular}{ l c{2} c{2} c{2} c{2} c{2} c{2} c{2} c{2} c{2} c{2} c{2} c{2} c{2} c{2} c{2} c{2}}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{ c c r r r r r r r r r r r r r r r r}
\toprule
\multirow{2}*{\textbf{Phase}} &\multirow{2}*{\textbf{\#Machines}} & \multicolumn{2}{c}{\textsc{als}} & \multicolumn{2}{c}{\textsc{bayes}} &\multicolumn{2}{c}{\textsc{gbt}} &\multicolumn{2}{c}{\textsc{km}} &\multicolumn{2}{c}{\textsc{lr}} &\multicolumn{2}{c}{\textsc{pca}} &\multicolumn{2}{c}{\textsc{rfc}} &\multicolumn{2}{c}{\textsc{svm}} \\
\cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}\cmidrule(lr){9-10}\cmidrule(lr){11-12}\cmidrule(lr){13-14}\cmidrule(lr){15-16}\cmidrule(lr){17-18}
 &  & Time & Cost & Time & Cost & Time & Cost & Time & Cost & Time & Cost & Time & Cost & Time & Cost & Time & Cost \\

\midrule

\cmidrule(lr){1-18}
% & 1 &  &  & 329.1 & 329.1 & 582.5 & 582.5 &  &  & 703 & 703 \\
% & 2 &  &  & 163.4 & 326.9 & 425.3 & 850.5 &  &  & 377.7 & 755.4 \\
% & 3 &  &  & 103.7 & 311 & 294.7 & 884.2 &  &  & 234.8 & 704.4 \\
% & 4 &  &  & 55.5 & 222.2 & 210.2 & 840.7 &  &  & 166.2 & 664.9 & & \\
 & 5 & x & x & 20.9 & 104.4 & 1545.1 & 7725.5 & 39.2 & 195.8 & 110.9 & 554.5 & 839.4 & 4197.0 & 120.8 & 604.1 & 141.3 & 706.5 \\
 & 6 & x & x & 16.5 & 99.1 & 243.8 & 1462.8 & 22.1 & 132.5 & 80.0 & 479.9 & 689.0 & 4134.2 & 98.5 & 591.3 & 111.4 & 668.4 \\
 & 7 & x & x & 13.7 & 96.2 & \cellcolor{green!100}\textbf{174.3} & \cellcolor{green!100}\textbf{1220.1} & \textbf{14.9}  & \textbf{104.3} & 63.3 & 442.9 & \cellcolor{green!100}\textbf{558.3} & \cellcolor{green!100}\textbf{3908.0} & \cellcolor{green!100}\textbf{80.9} & \cellcolor{green!100}\textbf{566.3} & 91.5 & 640.4 \\
 & 8 & x & x & 11.0 & 88.2 & \cellcolor{green!100}167.1 & \cellcolor{green!100}1336.8 & \cellcolor{green!100}4.6 & \cellcolor{green!100}36.4 & 43.7 & 350.0 & \cellcolor{green!100}511.0 & \cellcolor{green!100}4088.3 & \cellcolor{green!100}78.6 & \cellcolor{green!100}628.9 & 44.9 & 389.0 \\
 & 9 & \cellcolor{green!100}\textbf{123.5} & \cellcolor{green!100}\textbf{1111.2} & 9.4 & 84.3 & \cellcolor{green!100}170.5 & \cellcolor{green!100}1534.5 & \cellcolor{green!100}4.3 & \cellcolor{green!100}39 & 24.6 & 221.5 & \cellcolor{green!100}528.4 & \cellcolor{green!100}4756.0 & \cellcolor{green!100}74.6 & \cellcolor{green!100}671.4 & 19.9 & 178.8 \\
 & 10 & \cellcolor{green!100}154.9 & \cellcolor{green!100}1549.4 & 7.3 & 72.6 & \cellcolor{green!100}150.4 & \cellcolor{green!100}15.4 & \cellcolor{green!100}3.2 & \cellcolor{green!100}31.8 & 22.0 & 220.5 & \cellcolor{green!100}473.3 & \cellcolor{green!100}4733.4 & \cellcolor{green!100}71.8 & \cellcolor{green!100}718 & \cellcolor{green!100}\textbf{16.0} & \cellcolor{green!100}\textbf{159.8} \\
 & 11 & \cellcolor{green!100}107.6 & \cellcolor{green!100}1138.5 & \cellcolor{green!100}\textbf{5.1} & \cellcolor{green!100}\textbf{56.1} & \cellcolor{green!100}137.4 & \cellcolor{green!100}1511.4 & \cellcolor{green!100}3.2 & \cellcolor{green!100}35.2 & 16.2 & 178.0 & \cellcolor{green!100}483.6 & \cellcolor{green!100}5319.4 & \cellcolor{green!100}76.7 & \cellcolor{green!100}843.9 & \cellcolor{green!100}15.0 & \cellcolor{green!100}165.2 \\
 & 12 & \cellcolor{green!100}116.1 & \cellcolor{green!100}1393.2 & \cellcolor{green!100}5.1 & \cellcolor{green!100}61.6 & \cellcolor{green!100}121.4 & \cellcolor{green!100}1456.8 & \cellcolor{green!100}3.1 & \cellcolor{green!100}36.9 & \cellcolor{green!100}\textbf{14.7} & \cellcolor{green!100}\textbf{176.3} & \cellcolor{green!100}432.8 & \cellcolor{green!100}5193.7 & \cellcolor{green!100}76.6 & \cellcolor{green!100}919.3 & \cellcolor{green!100}13.8 & \cellcolor{green!100}166.2 \\
 \cmidrule(lr){1-18}
 Scale &  &  \multicolumn{2}{c}{\SI{e3}{\percent} (56.0 GB)}  & \multicolumn{2}{c}{\SI{150}{\percent} (26.4 GB)} &  \multicolumn{2}{c}{\SI{18e4}{\percent} (53.7 GB)} & \multicolumn{2}{c}{\SI{200}{\percent} (43.0 GB)}  &  \multicolumn{2}{c}{\SI{200}{\percent} (44.7 GB)}  &  \multicolumn{2}{c}{\SI{5e3}{\percent} (74.8 GB)}  &  \multicolumn{2}{c}{\SI{200}{\percent} (59.6 GB)} &  \multicolumn{2}{c}{\SI{150}{\percent} (89.4 GB)} \\
 \cmidrule(lr){1-18}
\bottomrule
\end{tabular}
\end{adjustbox}
\vspace{-10pt}}
\end{table*}
